SPS Beam Dump Facility -- Comprehensive Design Study

The proposed Beam Dump Facility (BDF) is foreseen to be located at the North Area of the SPS. It is designed to be able to serve both beam dump like and fixed target experiments. The SPS and the new facility would offer unique possibilities to enter a new era of exploration at the intensity frontier. Possible options include searches for very weakly interacting particles predicted by Hidden Sector models, and flavour physics measurements. In the first instance, exploitation of the facility, in beam dump mode, is envisaged to be for the Search for Hidden Particle (SHiP) experiment. Following the first evaluation of the BDF in 2014-2016, CERN management launched a Comprehensive Design Study over three years for the facility. The BDF study team has since executed an in-depth feasibility study of proton delivery to target, the target complex, and the underground experimental area, including prototyping of key sub-systems and evaluations of the radiological aspects and safety. A first iteration of detailed integration and civil engineering studies have been performed in order to produce a realistic schedule and cost. This document gives a detailed overview of the proposed facility together with the results of the studies, and draws up a possible road map for a three-year Technical Design Report phase, followed by a 5 to 6 year construction phase.

==> Beam_latex_tables/efficiencies_2018.tex <==
\begin{tabular}{lcc}
\toprule
{} &  TCC2 &  BDF/SHiP \\
\midrule
Extraction transmission            &  0.99 &      0.99 \\
TT20 transmission                  &  0.96 &      0.96 \\
Splitting transmission             &  0.80 &      1.00 \\
Total transmission                 &  0.76 &      0.95 \\
Protons per cycle [1e13]           &  2.50 &      4.20 \\
Effective protons per spill [1e13] &  1.90 &      3.99 \\
\bottomrule
\end{tabular}


==> Beam_latex_tables/hours_future_with-ion-run-4p9s-FT.tex <==
\begin{tabular}{l|ccccccccccc|cc}
\toprule
{} & Scheduled [hours] &  Effective [hours] \\
\midrule
Physics                    &           1,852.0 &            1,389.0 \\
Physics with parallel MD   &           1,356.0 &            1,017.0 \\
HiRadMat                   &             240.0 &              180.0 \\
AWAKE with parallel MD     &             265.5 &              199.1 \\
AWAKE                      &             742.5 &              556.9 \\
Dedicated MD               &             370.0 &              277.5 \\
Thursday MD                &             250.0 &              187.5 \\
Scrubbing                  &              72.0 &               54.0 \\
LHC setup (10\% of time)   &                 - &              514.8 \\
LHC filling (15\% of time) &                 - &              772.2 \\
Total                      &           5,148.0 &            5,148.0 \\
\bottomrule
\end{tabular}


==> Beam_latex_tables/supercycle_2018_TCC2-and-BDF-SHiP.tex <==
\begin{tabular}{l|ccccccccccc|cc}
\toprule
{} & \rot{AWAKE} & \rot{BDF/SHiP} & \rot{HiRadMat} & \rot{LHC filling} & \rot{LHC pilot} & \rot{MD dedicated} & \rot{MD parallel} & \rot{Scrubbing} & \rot{TCC2} & \rot{Zero} & \rot{Degauss} & \rot{Length [s]} & \rot{Power [MW]} \\
\midrule
AWAKE                    &           2 &              4 &              - &                 - &               - &                  - &                 - &               - &          1 &          - &             1 &             57.6 &            34.25 \\
AWAKE with parallel MD   &           2 &              3 &              - &                 - &               - &                  - &                 1 &               - &          1 &          - &             1 &             57.6 &            30.56 \\
Dedicated MD             &           - &              - &              - &                 - &               - &                  1 &                 - &               - &          - &          - &             - &             22.8 &            16.83 \\
HiRadMat                 &           - &              4 &              1 &                 - &               - &                  - &                 - &               - &          - &          - &             - &             51.6 &            25.58 \\
LHC filling              &           - &              2 &              - &                 1 &               - &                  - &                 - &               - &          - &          - &             - &             37.2 &            22.90 \\
LHC setup                &           - &              5 &              - &                 - &               1 &                  - &                 - &               - &          - &          - &             - &             48.0 &            32.29 \\
Physics                  &           - &              4 &              - &                 - &               - &                  - &                 - &               - &          1 &          - &             1 &             43.2 &            35.26 \\
Physics with parallel MD &           - &              4 &              - &                 - &               - &                  - &                 1 &               - &          1 &          - &             - &             46.8 &            32.64 \\
Scrubbing                &           - &              - &              - &                 - &               - &                  - &                 - &               1 &          1 &          - &             - &             33.6 &            28.39 \\
Thursday MD              &           - &              2 &              - &                 - &               - &                  1 &                 - &               - &          1 &          - &             1 &             51.6 &            27.89 \\
\bottomrule
\end{tabular}


==> Chapters/RoadMap/RoadMap-v0.tex <==
\chapter{Road Map}
\section{Status}

In 2016 the BDF team were charged by CERN management to complete key technical feasibility studies of the proposed facility in time for the ESPP update process.
This was in conjunction with a recommendation by the CERN Research Board to the SHiP experiment to prepare a Comprehensive Design Study as input to the ESPP update. 
Material and personnel resources were made available to perform in-depth studies and prototyping.
The key areas addressed were:  extraction and beam transfer; the target and target complex; radiation protection; safety engineering; integration; and civil engineering. 

Since inception, there has been sustained effort with good progress on all fronts as described in detail in this report. 
In brief, the study has addressed all pertinent technological challenges,
and in-depth studies and prototyping have been performed, or are already well underway, for all critical components and systems.
Through a mixture of novel hardware development, beam physics and technology, the study and prototype validation
have shown that SPS can deliver the beam with the required characteristics, with acceptable losses, to a robust target housed in a functional and secure target complex. The radiological implications appear manageable, 
The technologies and their deployment,  although challenging, appear to be within CERN's established competencies,
and the project, given the resources, is ready to move towards the detailed design and execution phase.



 
% Markus Brugger: This could be effectively addressed by combining the BDF shutdown work with a Phase-1(a) of the NA-CONS project, addressing the work required in TCC2/TDC2. As discussed/proposed in the IRRC, the required resources could be balanced with a 2y stop not only of the NA, but also the SPS. Saying this, a proposed modification of the above paragraph could be: “the main challenge for BDF will be to optimize the scheduling of the CE works to minimise the impact on SPS NA operation, since the full works cannot be accommodated in the currently foreseen 12 month LS3 shutdown. A respective extension to 24 months would also be beneficial to address important consolidation requirements of the overall SPS NA complex.”
 


\section{Feasibility study phase}

The feasibility study phase will come to an end with the delivery of this Comprehensive Design Study which is timed to coincide with the ESPP update process.

With the go ahead from CERN management, under the continuing auspices of Physics Beyond Colliders,
it is foreseen to continue these studies in 2019 and 2020.
Specific areas include:
\begin{itemize}
    \item Post Irradiation Examination (PIE) of the prototype target tested in 2018;
    \item helium vessel design and preparation for prototyping;
    \item construction and testing of the prototype laminated switch/splitter magnet;
    \item intermediate iteration of system integration;
    \item development and possible prototyping of the hadron absorber magnetisation system;
    \item continued studies of loss reduction techniques during slow extraction in the SPS and the deployment of these techniques onto operational beams (planned for the SPS run starting in 2021); 
    \item site investigation required for a definitive civil engineering study. 
\end{itemize}

\section{Studies during the TDR phase}

By the end of 2020, the BDF team would hope to be in a position to seek approval to go ahead with the
preparation of a technical design report (TDR).
While working towards the delivery of a TDR, it is envisioned to perform:
\begin{itemize}
    \item detailed engineering studies and specification of the deliverables for
    both standard and novel systems;
    \item  detailed integration plans;
    \item civil engineering pre-construction activities i.e.
    environmental impact study; build permit submission/approval; tender process and detailed civil engineering  design;
    \item definitive radiation protection studies.
\end{itemize}
The completion of these activities would lead to the delivery of the TDR in 2022.
The aim would be to seek project approval in 2023, allowing subsequent project execution to take advantage of the North Area stop during LS3. 

A summary of the possible evolution of the BDF project is shown in Table \ref{tab:time-line}.

\begin{table}[h]
\begin{center}
\caption{Outline of a possible BDF time-line}
\label{tab:time-line}
\begin{tabular}{|l|l|}
\hline
2017 - 2018 & Prototyping of key technologies \\
 & Preliminary infrastructure integration \& CE designs \\
 & Preliminary Cost estimates and schedule \\
 \hline
Start 2019  & Delivery of Comprehensive Design Study \\
\hline
2019 - 2020 & Continued design studies and prototyping \\
\hline
End 2020 & Approval to go ahead with TDR \\
\hline
2021 - 2022  & Engineering design studies towards TDR \\
 & Detailed integration studies \\
 & Specification towards production  \\
 & CE pre-construction activities (environmental impact study; \\
 & build permit submission/approval; detailed CE design and pre-tender process) \\
 \hline
2022  & TDR delivery \\
\hline
 2023 & Seek approval \\
 2023+ &  Tender, component production, CE contracts  \\
\hline
\end{tabular}
\end{center}
\end{table}

Some further investigation work as detailed in the Civil Engineering chapter will need to be carried out before detailed civil engineering design can begin with specialist external consultancies. Once these designs are complete, tendering for the civil construction contracts can start. 

In parallel, an environmental impact study must be prepared and approved by the local authorities, prior to the timely submission of the building permit application for the project, to allow construction works to commence. 




\subsection{Civil Engineering Schedule and Resource Considerations} \label{programme}

The Civil Engineering work is split into four main packages, as indicated within Fig. \ref{fig:Workpackages}.  

\begin{figure}[ht]
\centering\includegraphics[width=.87\linewidth]{Figures/CivEng/Workpackages.jpg}
\caption{Indicative division and sequence of work packages for delivery of BDF project}
\label{fig:Workpackages}
\end{figure}

WP1, WP2 and WP3 activities can all start after detailed design and tendering of works is complete (construction works can be performed during normal beam operation in the North Area, where the only constraint is a requirement to maintain 8 m of earth shielding to TCC2 given by Radiation Protection considerations). 

In principle, these work packages can be partially executed in parallel, although this needs to be studied in more detail and carefully set out in contract documents to avoid cost increases from contractors working in close proximity to one another. Various activities including access roads, technical galleries and other non-area specific tasks have been included as miscellaneous works and are not assigned specifically to any work package. It is likely these activities will need to be done as advanced enabling works or as part of the first work package.

WP4 includes all the activities that must be carried out during beam stop which is likely to be during Long Shutdown 3 (LS3). This will include the junction cavern demolition and reconstruction along with the construction of the extraction tunnel up to a point where the distance between proposed extraction tunnel and TCC2 reduces to \SI{8}{\metre}. The current beam operation schedule includes approximately 12 months of beam shut-down. This is  unlikely to be sufficient to carry out the required civil engineering works. Other activities such as the machine and tunnel cool-down, infrastructure dismantling/ re-installation and testing/ commissioning must also be considered in the works schedule in order to calculate the required period of North Area shutdown. 

The key drivers of the construction phase are outlined below.

\begin{itemize}
    \item  { \bf Civil engineering underground works} are estimated to take 2.75 years:
    
 \begin{itemize}
     \item 1.25 years for the re-construction of junction cavern and the construction of the first of the new transfer line (WP4)
     \item 1.25 years for the final part of the new transfer line and access shafts (WP3)
     \item 1.0 year for the target complex (WP2)
     \item 1.25 years for the detector hall  (WP1)
 \end{itemize}  
 Figures shown without contingency. 
 Radiological considerations have been taken into account.
The re-construction of the junction cavern and construction of the first part of the 
new transfer line will take around 1.5 years (with contingency) and, as noted above, precludes North Area operation in parallel.  
This work package should be timed to coincide with a long shutdown of the SPS to minimise the impact on North Area users. The work requires a period of cool down after the stop of North Area operation, which could be largely covered by a preceding ion run.
The other major civil engineering works
(final section of new transfer line, Target Complex, Experimental Hall)
can be executed in parallel with North Area operation. 
\vspace{4 mm}
    
    \item {\bf Civil engineering surface works }, following on from the associated underground works, are estimated to take 1.75 years:
    
 \begin{itemize}
     \item 0.75 year for access building and auxiliary building
     \item 1.0 year for service building and target
     \item 1.0 year for the detector hall
 \end{itemize}   
    These work packages can be executed in parallel with underground work where appropriate.
\vspace{4 mm}    
    \item {\bf Installation} can be staged as the given structures become available.
    \begin{itemize}
    \item Re-installation of junction cavern hardware and services
    \item Installation of hardware and services on new beamline
    \item Installation of hardware and services in the target hall
    \item Service building hardware, services, access and safety systems
    \item For the Experimental hall, the entire installation phase is expected to take 2--2.5 years.
    \end{itemize}

\end{itemize}


\subsection{Schedule}

The medium-term schedule (circa 2019) of the injector complex and the LHC, foresees long shutdowns for the injectors in 2019-2020 (LS2) and 2025 (LS3). 
LS3 for the LHC stretches from 2024 to mid-way through 2026.

A preliminary schedule has been studied for the construction of the BDF facility using the knowledge acquired from the construction of previous similar schemes at CERN. This timeline is shown in Fig. \ref{fig:Schedule}. 

\begin{figure}[ht]
\centering\includegraphics[width=.87\linewidth]{Figures/CivEng/Schedule.png}
\caption{Indicative draft schedule for CE implementation showing existing LHC and SPS schedules along with required additional north area stoppage.}
\label{fig:Schedule}
\end{figure}



==> Cost-tables/CV-summary.tex <==
\begin{tabular}{llc}
\hline
 &  & kCHF \\
\hline
Target complex & Cooling & 1863 \\
Target complex & Ventilation & 1616 \\
Extraction tunnel + service building & Cooling & 3657 \\
Extraction tunnel + service building & Ventilation & 1202 \\
Experimental hall & Cooling  & 828 \\
Experimental hall & Ventilation  & 2622 \\
\hline
TOTAL   &  & 11788 \\
\hline

\end{tabular}

==> Cost-tables/TTC-MPE.tex <==
\begin{tabular}{lll}
\hline
Item &  	Staff  &	Fellows   \\
		 &	[FTE] &	 [MCHF] & \\
	\hline
	Target assembly \& annex equipment 	 &	15 &		0.9	\\
	Instrumentation package 	 &	5 &		0.45  \\
	Bunker iron shielding \& US1010  &		3 &		0.6	  \\
	Concrete shielding 	 &	3 &		0	  \\
	Magnetized coil for US1010 shield 	 &	3 &		0.3  \\
	Target \& coil handling system  &		25 &		1.8 \\
	Target and coil shielding casks	  &		0.5 &		0  \\
	Helium vessel (HW)  &		11 &		0.6  \\
	Integration	 	 &	6 &		0  \\
	Beam window(s)	  &	2 &		0.3  \\
	Survey \& alignment	 x	 &	3	 &	0.3	  \\
	Collimator(s) 	 &	0.5	 &	0.15  \\
\hline					
		TOTAL  &		77.0 &		5.4	 \\
\hline
\end{tabular}

==> Cost-tables/TTC-summary.tex <==
\begin{tabular}{lll}
\hline
Item &  Material   &	Comments \\
		 & [MCHF]  & \\
	\hline
	Target assembly \& annex equipment &		5.6	  & extrapolated from target proto  \\
	Instrumentation package &	 	0.9	 &		Best guess based on recent activities \\
	Bunker iron shielding \& US1010 &		14.0 &		Cost based on recent contracts \\
	Concrete shielding &		0.8	 &		Cost based on recent contracts \\
	Magnetized coil for US1010 shield &		1.0	 &			Guess \\
	Target \& coil handling system &		19.1 &	OTL study CERN-699-TNT-015-C \\
	Target and coil shielding casks	 &	0.2 &		Best guess based on recent activities \\
	Helium vessel (HW) &		2.3 &			Best guess based on recent activities \\
	Integration	 &	0.6	 &		Guess \\
	Beam window(s)	 &	0.6	 &			Guess \\
	Survey \& alignment	 &	0.5	 &		Guess \\
	Collimator(s) &		0.5	 &		Best guess based on recent activities \\
\hline					
		TOTAL &		46.0 &	 \\
\hline
\end{tabular}

==> CostSections/civil-engineering.tex <==

%\section{Civil Engineering}

\subsubsection{Basis of estimate}

The cost estimate for the BDF Project has been based on the layouts presented in the civil engineering chapter. The estimate produced includes all aspects of construction, detailed engineering design work and construction management except where stated otherwise. Many of the rates used to formulate this estimate have been based on real construction costs from the large hadron collider experience (1998-2005), from consultant (ILF's) future circular collider cost studies \cite{ILF} and following recent tendering for similar projects at CERN such as CENF and HiLumi. In addition to this process, ARUP have independently reviewed the cost estimate as part of their scope of work and the results have been fed back into the costing process to ensure a robust estimate. 

The civil engineering activities have been split into four primary work packages as shown in the chapter discussing the BDF Roadmap. 
The provisional cost for the main tasks identified and included within each package is shown in the summary table \ref{tab:CECosts}.

\begin{table}[htb]
\begin{center}
\caption{Summary cost estimates for the CE work packages}
\label{tab:CECosts}
\begin{tabular}{ll}
\hline\hline
Work package & Cost [MCHF]      \\
\hline	
Work Package 1  & 	31.7 \\
Work Package 2 & 	16.5 \\
Work Package 3 & 	10.9 \\
Work Package 4  & 	7.3 \\
Work Package 5  & 	1.3 \\
Site investigation  & 	0.6 \\
\hline
Facility total & 	68.3 \\
\hline\hline
\end{tabular}
\end{center}
\end{table}

The accuracy of the estimate is considered Class 4 - Study or Feasibility which could be 15-\SI{30}{\percent} lower or 20-\SI{50}{\percent} higher (in line with AACE international's best practice recommendations \cite{christensen} as has been used for previous CERN projects). Until the project requirements are further developed, it is suggested that a suitable band to adopt would be \SI{-20}{\percent} to +\SI{40}{\percent} for CE costs.



\subsubsection{Costing assumptions and exclusions}

The cost estimate is based on the following assumptions:

\begin{itemize}
\item Costs have been based on retaining spoil on CERN land with no tipping and disposal costs. If this were to change, the cost increase would be significant.
\item The proposed drainage can be connected into existing drainage without significant capacity enhancement of the existing.
\item Build up of hardstanding areas and access road can be carried out using site won material with only 1.5\,m depth road construction.
\item Radiation protection measures required for the works and assumptions agreed are as stated in \cite{ARUP2018-1,ARUP2018-2}.
\item The construction works programme will be as stated in the schedule as noted in the BDF roadmap chapter. This programme is outline and will need to be reviewed to optimise activities to allow multiple work packages to progress in parallel. 
\item Ground and groundwater conditions do not vary significantly from those previously found in the area.
\item No improvements are required to the wider Pr\'{e}vessin site for office space, restaurant, main access, road network etc
\item Building 687 will be demolished and a replacement constructed elsewhere while de-mountable buildings 6357 and 6575 and a container - 6361, will be relocated. An area of hardstanding will be re-provided to replace the existing.
\item Assumptions have been made on the required depth of diaphragm walling, however the cost is very sensitive to changes in depth due to the large proportion of total scheme costs relating to diaphragm wall construction (approx. 27\%).
\item Allowances have been made for temporary propping of TCC2 and excavations during diaphragm wall construction, however this will depend on ground conditions meaning they are subject to change.
\item An allowance has been made for four tensile fabric structures to temporarily house activated soil before re-use with two thirds of material re-used directly without intermediate storage. 
\end{itemize}

All temporary facilities needed for the civil engineering works have been included in the cost estimate, but nothing for any temporary areas/buildings needed for machine or detector assembly/installation. 

For clarity, the overall cost estimate does not include:

\begin{itemize}
\item SMB-SE Resources 
\item Special foundation support for facilities (e.g. Detector, etc) 
\item Shielding precast concrete blocks 
\item Infrastructure and services costs eg heating, ventilation, cooling, electricity, gas etc
\item Tenting over excavation and demolition of TDC2

\end{itemize}

\subsubsection{Spend profile}

The annual cost forecast is indicated in Fig.~\ref{fig:Spendprofile}. The cost per year has been split between the``civil engineering works'' related to the construction phase and initial site investigation and the ``expert assistance'' which covers the entire civil engineering process. 

\begin{figure}[ht]
\centering\includegraphics[width=.87\linewidth]{Figures/BDFCosts/Spendprofile.png}
\caption{Indicative annual spend profile for CE works.}
\label{fig:Spendprofile}
\end{figure}



==> TC-Sections/CV_Files/CFD_HeVessel_Short.tex <==
CFD simulations for the helium vessel have been run in support of the helium vessel design effort. The purpose of these simulations is to confirm that helium circulates properly in the helium vessel, and that the following general constraints are met:
\renewcommand{\labelenumi}{\Alph{enumi}.}
\begin{enumerate}
\item During start-up of the helium passivation system, the formation of air pockets shall be prevented so that the air-to-helium replacement procedure happens smoothly. This constraint will help to minimize the amount of pure helium lost to the atmosphere during the air-helium mixture flushing; it will also minimize the overhead on the helium purification system during the purification phase of the start-up procedure;
\item During operation of the helium passivation system, the helium flow stagnation areas shall be minimized. This constraint will help to minimize the amount of impurities remaining in the helium vessel (not treated by the helium purification system), thus reducing the potential activation of the gas mixture.
\end{enumerate}

Two sets of simulations have been run, a steady-state case simulating the nominal helium circulation through the vessel, and a transient case simulating the start-up of the system via flushing.

\subsubsection{3D Model} 
 
Figure \ref{Fig:TC:BDF_HeVe_3Dout} shows a view of the 3D model for the helium vessel, after model clean-up. A series of ribs supports the steel containment on each face. For the purpose of this simulation, the lid is provided with six cylindrical penetrations (70 mm each) that represent the helium supply and distribution system; the final design of the helium vessel will be provided with a single penetration on one of the side faces and an internal distribution system that replicates the function of these six inlets. Similarly, the outlet is represented by three cylindrical penetrations at the bottom-left corner in Figure \ref{Fig:TC:BDF_HeVe_3Dout}. Figure \ref{Fig:TC:BDF_HeVe_3Dout} also shows the penetration and the door for the trolley that supports the target and allows its insertion and extraction from the helium vessel. \hl{Figure 1} shows a view of the internal components of the helium vessel.

\begin{figure}[htbp]
\centering % 
\includegraphics[width=1\linewidth]{Figures/TargetComplex/CV_Figures/HeVeCFD_010.png}
\caption{\label{Fig:TC:BDF_HeVe_3Dout} 3D model of the helium vessel}
\end{figure}

\subsubsection{Mesh} 

The size of the model and the presence of a high number of thin volumes make the meshing process relatively challenging. The mesh has been developed using Fluent Meshing, and the CFD surface mesh approach. The gaps between blocks have been grown using prism meshing, in order to create cells with high aspect-ratio. Figure \ref{Fig:TC:BDF_HeVe_Mesh1} shows a mesh slice in the collimator-target region and Table \ref{Tab:TC:BDF_HeVe_MeshStat} shows the mesh statistics.

\begin{figure}[htbp]
\centering % 
\includegraphics[width=1\linewidth]{Figures/TargetComplex/CV_Figures/HeVeCFD_020.png}
\caption{\label{Fig:TC:BDF_HeVe_Mesh1} Mesh slice in the collimator-target region}
\end{figure}

\begin{table}[htbp]
\centering
\caption{\label{Tab:TC:BDF_HeVe_MeshStat} Mesh statistics}
\smallskip
\begin{tabular}{l|r|l}
\hline
\textbf{Parameter} & \textbf{Value} & \textbf{Unit}\\
\hline
Size & 6782628 & cells \\
Allocated memory & 10982 & Mbytes \\
Total volume & 74.5 & m3 \\
Min. orthogonal quality & 3.34 & \%\\
Max. aspect-ratio & 328 & -\\
Mesh check & Passed & -\\
\hline
\end{tabular}
\end{table}

\subsubsection{Helium Circulation Simulation}

A steady-state simulation of helium circulation has been run to analyze the pressure and velocity distributions and to identify locations where helium velocity is particularly small.
The flow rate selected for the simulation, 764.45 m3/h, represents the flow provided by the cooling compressor of the helium passivation system; note that the design flow of the purification part of the helium passivation system is much smaller, 75 m3/h.
The primary intent of the steady simulation is the identification of areas where the flow velocity is close to 0 m/s (stagnant flow). Excluding the inlet and outlet locations (where velocity is well beyond 20 cm/s), the velocity distribution generally looks uniform and not higher than 10 cm/s. In order to show areas of low velocity, the scale has been reduced to a maximum velocity of 0.1 mm/s, corresponding to 6 mm/min. Figure \ref{Fig:TC:BDF_HeVe_Steady1} shows a vector plot colored by velocity magnitude and clipped to 0.1 mm/s. The figure shows that the main critical areas are the trolley, the target the proximity shielding and the collimator assembly. Note that the areas identified in the upper and lower plenum are not as critical because they are located in open volumes, for which recirculation and gravity would help providing some mixing effect.

\begin{figure}[htbp]
\centering % 
\includegraphics[width=1\linewidth]{Figures/TargetComplex/CV_Figures/HeVeCFD_030.png}
\caption{\label{Fig:TC:BDF_HeVe_Steady1} Vector plot colored by velocity magnitude and clipped to 0.1 mm/s}
\end{figure}

\subsubsection{Flushing Simulation}

A transient simulation of the helium filling process has been run to identify air pockets that remain in the helium vessel during the flushing. The setup of the simulation is analogous to the steady-state simulation, except for the fact that the initial condition is a vessel filled of air and the inlet supplies pure helium. The total simulation time is equivalent to 166.5 m3 of pure helium injected at 764.45 m3/h; since the helium vessel free volume is 74.5 m3, the mentioned pure helium amount is equivalent to 2.23 gas changes.

Figure \ref{Fig:TC:BDF_HeVe_Tr1} shows a volume rendering of the helium mole fraction (helium purity) distribution in the helium vessel at six instants of time during the transient. As a reference, the last snapshot of the series (8 minutes and 34 seconds) corresponds to about 1.46 volumes of pure helium injected in the system. The series of plots shows that the helium flow gradually and uniformly fills the helium vessel, including its gaps, from top to bottom. The 764.45 m3/h flow rate has been selected because it is expected to be more critical than a lower flow rate (such as the purification flow rate) in terms of helium-air mixing: high velocity and high turbulence should enhance mixing between the two gases, thus increasing the time needed for flushing and the amount of pure helium lost. However the results of the simulation seem to contradict this expectation; factors that may influence this behavior are the complicated geometry, which enhances separation between helium and air, and mixing by diffusion, which has a smaller impact on small time scales.

\begin{figure}[htbp]
\centering % 
\includegraphics[width=1\linewidth]{Figures/TargetComplex/CV_Figures/HeVeCFD_040.png}
\caption{\label{Fig:TC:BDF_HeVe_Tr1} Volume rendering of helium mole fraction during filling}
\end{figure}

Figure \ref{Fig:TC:BDF_HeVe_Tr2} shows the helium purity evolution with time. The three datasets represent the following quantities:
\begin{itemize}
\item Injected volume fraction: volume of pure helium injected in the vessel, normalized by the vessel free volume (74.5 m3); this parameter is useful to identify the number of gas changes: it reaches 1.0 when one volume change has been achieved. Since 1.0 is achieved at about 350 s, 2 volume changes (threshold for pure helium loss) are achieved at about 700 s; 
\item Outlet average fraction: surface average helium purity (weighted by mass) at the outlets of the helium vessel. This is the purity that would be measured by a purity meter at the inlet of the purification system. Note that the peak at ~615 s is not physical (generated by local convergence issues during the simulation) and should be disregarded;  
\item Volume average fraction: average helium purity in the helium vessel as function of time.
\end{itemize}

The parameter of interest is the volume average fraction or purity. The flushing process allows to reach a high purity without losing a large amount of helium before being able to start the purification process: the volume average fraction reaches 85\% (threshold for purification system) at about 350 s, equivalent to about 1 volume change (Injected volume fraction equal to 1). The behavior of the volume average fraction is asymptotically increasing to 1; the average purity is 85\% at 1 volume change and >98\% at 2 volume changes (~700 s). The outlet average fraction is delayed (due to the inertia of the system) and more oscillating; it consistently exceeds 90\% only towards the end of the second volume change.

\begin{figure}[htbp]
\centering % 
\includegraphics[width=1\linewidth]{Figures/TargetComplex/CV_Figures/HeVeCFD_050.png}
\caption{\label{Fig:TC:BDF_HeVe_Tr2} Helium mole fraction as function of time}
\end{figure}

Figure \ref{Fig:TC:BDF_HeVe_Tr3} represents helium purity at different locations in the helium vessel at the end of the simulated transient, corresponding to 13 min and 4 sec, or 2.23 volume changes; the scale is clipped to a maximum purity of 98.5\% to show areas of low purity. The minimum purity is about 82\% and it is likely located in the collimator area. Not many low-purity areas are identified, proving that the current design provides good circulation patterns for helium. Note that the large impurity volume located in the lower plenum should be neglected since it would naturally disappear with a longer simulation time.

\begin{figure}[htbp]
\centering % 
\includegraphics[width=1\linewidth]{Figures/TargetComplex/CV_Figures/HeVeCFD_060.png}
\caption{\label{Fig:TC:BDF_HeVe_Tr3} Vector plot of helium mole fraction clipped at 98.5\% (2.23 volume changes)}
\end{figure}

\subsubsection{Recommendations}

The following conclusions and recommendations can be listed following a preliminary simulation analysis:
\begin{itemize}
\item The presence of a 10 mm gap between blocks and vessel internals provides an acceptable level of helium purity after flushing, even at high inlet flow rate;
\item The current design allows to achieve 85\% average purity (minimum required to start the purification system) in the helium vessel well before reaching 2.0 pure helium volume changes;
\item 2.0 volume changes are recommended before starting the helium purification system, so that not only the volumetric average purity, but also the outlet surface average purity is beyond 85\%; 
\item The control over the accuracy of gap thicknesses is important to prevent the formation of unexpected stagnation areas or flow imbalances. This is particularly true for the lateral concrete shielding blocks, or any location where a bypass flow could be generated by unplanned variation of gap sizes, leaving some areas unventilated;
\item The presence of corners combined with horizontal gaps generally makes stagnation areas more likely to appear;
\item Horizontal gaps with large surface should be avoided as much as possible; if this is not possible, the dimensions and geometry of the gap shall be defined and a CFD analysis shall prove that stagnation is limited as much as possible.
\end{itemize}
